Practical application of the multi-model approach in the study of complex systems

Different kinds of models are used to study various natural and technical phenomena. Usually, the researcher is limited to using a certain kind of model approach, not using others (or even not realizing the existence of other model approaches). The authors believe that a complete study of a certain phenomenon should cover several model approaches. The paper describes several model approaches which we used in the study of the random early detection algorithm for active queue management. Both the model approaches themselves and their implementation and the results obtained are described.

==> bib/red-model-approach/bibtool/include/doi <==
# Convert URL DOI to DOI
#rewrite.rule = {url# "https?://.*doi"} # Should have DOI field instead
#rewrite.rule = {url# "https?://.*doi\.org/\(10\.[0-9]+/[^\"}]+\)" # "{\1}"}
rename.field {url=doiurl if url="doi"}
rename.field {doiurl=delete if doi="10."}
delete.field = {delete}
rename.field {doiurl=doi}
rewrite.rule = {doi# "https?://.*doi\.org/\(10\.[0-9]+/.+\)"# "\1"}


==> bib/red-model-approach/bibtool/include/month <==
#
# This resource file tries to introduce BibTeX strings for month names.
# Provisions are made to preserve other information contained in the
# month field.
#

rewrite.rule { month = "^[\"{] *\(.*\)january\(.*\) *[\"}]$" # "{\1} # 1 # {\2}" }
rewrite.rule { month = "^[\"{] *\(.*\)february\(.*\) *[\"}]$" # "{\1} # 2 # {\2}" }
rewrite.rule { month = "^[\"{] *\(.*\)march\(.*\) *[\"}]$" # "{\1} # 3 # {\2}" }
rewrite.rule { month = "^[\"{] *\(.*\)april\(.*\) *[\"}]$" # "{\1} # 4 # {\2}" }
rewrite.rule { month = "^[\"{] *\(.*\)may\(.*\) *[\"}]$" # "{\1} # 5 # {\2}" }
rewrite.rule { month = "^[\"{] *\(.*\)june\(.*\) *[\"}]$" # "{\1} # 6 # {\2}" }
rewrite.rule { month = "^[\"{] *\(.*\)july\(.*\) *[\"}]$" # "{\1} # 7 # {\2}" }
rewrite.rule { month = "^[\"{] *\(.*\)august\(.*\) *[\"}]$" # "{\1} # 8 # {\2}" }
rewrite.rule { month = "^[\"{] *\(.*\)september\(.*\) *[\"}]$" # "{\1} # 9 # {\2}" }
rewrite.rule { month = "^[\"{] *\(.*\)october\(.*\) *[\"}]$" # "{\1} # 10 # {\2}" }
rewrite.rule { month = "^[\"{] *\(.*\)november\(.*\) *[\"}]$" # "{\1} # 11 # {\2}" }
rewrite.rule { month = "^[\"{] *\(.*\)december\(.*\) *[\"}]$" # "{\1} # 12 # {\2}" }

rewrite.rule { month = "^[\"{] *\(.*\)jan\(.*\) *[\"}]$" # "{\1} # 1 # {\2}" }
rewrite.rule { month = "^[\"{] *\(.*\)feb\(.*\) *[\"}]$" # "{\1} # 2 # {\2}" }
rewrite.rule { month = "^[\"{] *\(.*\)mar\(.*\) *[\"}]$" # "{\1} # 3 # {\2}" }
rewrite.rule { month = "^[\"{] *\(.*\)apr\(.*\) *[\"}]$" # "{\1} # 4 # {\2}" }
rewrite.rule { month = "^[\"{] *\(.*\)may\(.*\) *[\"}]$" # "{\1} # 5 # {\2}" }
rewrite.rule { month = "^[\"{] *\(.*\)jun\(.*\) *[\"}]$" # "{\1} # 6 # {\2}" }
rewrite.rule { month = "^[\"{] *\(.*\)jul\(.*\) *[\"}]$" # "{\1} # 7 # {\2}" }
rewrite.rule { month = "^[\"{] *\(.*\)aug\(.*\) *[\"}]$" # "{\1} # 8 # {\2}" }
rewrite.rule { month = "^[\"{] *\(.*\)sep\(.*\) *[\"}]$" # "{\1} # 9 # {\2}" }
rewrite.rule { month = "^[\"{] *\(.*\)oct\(.*\) *[\"}]$" # "{\1} # 10 # {\2}" }
rewrite.rule { month = "^[\"{] *\(.*\)nov\(.*\) *[\"}]$" # "{\1} # 11 # {\2}" }
rewrite.rule { month = "^[\"{] *\(.*\)dec\(.*\) *[\"}]$" # "{\1} # 12 # {\2}" }

rewrite.rule { month = "^{ *} # " = ""}
rewrite.rule { month = " # { *}$" = ""}


==> image/red-model-approach/en/Makefile <==
PLANTUML_FIG := $(wildcard *.pu)
pdf_files := $(patsubst %.pu, %.pdf, $(PLANTUML_FIG))

all: $(pdf_files)

clean:
	-rm -f *.{log,toc,tac,aux,dvi,ps,bbl,blg,tmp,nav,out,snm,vrb,rel,thm,rel,*~} *eps-converted-to.pdf *.synctex.gz
	-rm -f split*
	rm -rf out auto
	for i in $(ALLSUBDIRS); do \
	    (cd $$i; make clean) || exit 1; \
	done

cleanall: clean
	-rm $(pdf_files)

%.svg : %.pu
	-plantuml -nbthread auto -tsvg $<

%.pdf : %.svg
	-rsvg-convert -d 600 -p 600 -u -f pdf $< -o $@


==> image/red-model-approach/ru/Makefile <==
PLANTUML_FIG := $(wildcard *.pu)
pdf_files := $(patsubst %.pu, %.pdf, $(PLANTUML_FIG))

all: $(pdf_files)

clean:
	-rm -f *.{log,toc,tac,aux,dvi,ps,bbl,blg,tmp,nav,out,snm,vrb,rel,thm,rel,*~} *eps-converted-to.pdf *.synctex.gz
	-rm -f split*
	rm -rf out auto
	for i in $(ALLSUBDIRS); do \
	    (cd $$i; make clean) || exit 1; \
	done

cleanall: clean
	-rm $(pdf_files)

%.svg : %.pu
	-plantuml -nbthread auto -tsvg $<

%.pdf : %.svg
	-rsvg-convert -d 600 -p 600 -u -f pdf $< -o $@

